Semantic Sensitivities and Inconsistent Predictions: Measuring the Fragility of NLI Models

Recent studies of the emergent capabilities of transformer-based Natural Language Understanding (NLU) models have indicated that they have an understanding of lexical and compositional semantics. We provide evidence that suggests these claims should be taken with a grain of salt: we find that state-of-the-art Natural Language Inference (NLI) models are sensitive towards minor semantics preserving surface-form variations, which lead to sizable inconsistent model decisions during inference. Notably, this behaviour differs from valid and in-depth comprehension of compositional semantics, however does neither emerge when evaluating model accuracy on standard benchmarks nor when probing for syntactic, monotonic, and logically robust reasoning. We propose a novel framework to measure the extent of semantic sensitivity. To this end, we evaluate NLI models on adversarially generated examples containing minor semantics-preserving surface-form input noise. This is achieved using conditional text generation, with the explicit condition that the NLI model predicts the relationship between the original and adversarial inputs as a symmetric equivalence entailment. We systematically study the effects of the phenomenon across NLI models for $\textbf{in-}$ and $\textbf{out-of-}$ domain settings. Our experiments show that semantic sensitivity causes performance degradations of $12.92\%$ and $23.71\%$ average over $\textbf{in-}$ and $\textbf{out-of-}$ domain settings, respectively. We further perform ablation studies, analysing this phenomenon across models, datasets, and variations in inference and show that semantic sensitivity can lead to major inconsistency within model predictions.

==> tables/drop_rate.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{@{}clcccccc|c@{}}
\toprule
                                                                                                  & \textbf{}                         & \textbf{bart-l} & \textbf{roberta-l} & \textbf{distilbart} & \textbf{deberta-b} & \textbf{deberta-l} & \textbf{deberta-xl} & Average                  \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\end{tabular}}}     & \multicolumn{1}{l|}{1st Dropping} & 90.10\%         & 90.56\%            & 87.17\%             & 88.77\%            & 91.32\%            & 91.44\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 88.89\%         & 89.24\%            & 86.13\%             & 87.07\%            & 89.69\%            & 90.28\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{1.20\%} & \textbf{1.31\%}    & \textbf{1.04\%}     & \textbf{1.70\%}    & \textbf{1.63\%}    & \textbf{1.16\%}     & \textbf{1.34\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}SNLI\end{tabular}}}    & \multicolumn{1}{l|}{1st Dropping} & 87.55\%         & 86.44\%            & 84.37\%             & 84.39\%            & 88.87\%            & 88.54\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 82.78\%         & 81.78\%            & 82.02\%             & 78.89\%            & 83.64\%            & 84.62\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{4.77\%} & \textbf{4.66\%}    & \textbf{2.35\%}     & \textbf{5.50\%}    & \textbf{5.23\%}    & \textbf{3.92\%}     & \textbf{4.41\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r1\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 46.20\%         & 46.40\%            & 41.40\%             & 35.10\%            & 49.70\%            & 53.00\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 45.60\%         & 44.90\%            & 41.10\%             & 34.30\%            & 48.60\%            & 52.00\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.60\%} & \textbf{1.50\%}    & \textbf{0.30\%}     & \textbf{0.80\%}    & \textbf{1.10\%}    & \textbf{1.00\%}     & \textbf{0.88\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r2\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 31.60\%         & 27.00\%            & 32.80\%             & 29.80\%            & 32.70\%            & 35.40\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 30.80\%         & 25.30\%            & 32.30\%             & 28.80\%            & 31.60\%            & 34.70\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.80\%} & \textbf{1.70\%}    & \textbf{0.50\%}     & \textbf{1.00\%}    & \textbf{1.10\%}    & \textbf{0.70\%}     & \textbf{0.97\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r3\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 33.08\%         & 26.75\%            & 32.75\%             & 30.50\%            & 35.92\%            & 38.75\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 32.67\%         & 26.33\%            & 32.17\%             & 29.58\%            & 35.42\%            & 38.08\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.42\%} & \textbf{0.42\%}    & \textbf{0.58\%}     & \textbf{0.92\%}    & \textbf{0.50\%}    & \textbf{0.67\%}     & \textbf{0.58\%}          \\ \midrule
\multicolumn{1}{l|}{Average}                                                                      &                                   &                 &                    &                     &                    &                    &                     & \textit{\textbf{1.64\%}} \\ \bottomrule
\end{tabular}
\caption{Proportion of instances left after each filter. On average, the second filter leads to $1.64\%$ instances of the full dataset getting dropped, which is negligible.}
\label{tab:dropprop}
\end{table*}
